Anomalous Sound Detection as a Simple Binary Classification Problem with Careful Selection of Proxy Outlier Examples

Unsupervised anomalous sound detection is concerned with identifying sounds that deviate from what is defined as 'normal', without explicitly specifying the types of anomalies. A significant obstacle is the diversity and rareness of outliers, which typically prevent us from collecting a representative set of anomalous sounds. As a consequence, most anomaly detection methods use unsupervised rather than supervised machine learning methods. Nevertheless, we will show that anomalous sound detection can be effectively framed as a supervised classification problem if the set of anomalous samples is carefully substituted with what we call proxy outliers. Candidates for proxy outliers are available in abundance as they potentially include all recordings that are neither normal nor abnormal sounds. We experiment with the machine condition monitoring data set of the 2020's DCASE Challenge and find proxy outliers with matching recording conditions and high similarity to the target sounds particularly informative. If no data with similar sounds and matching recording conditions is available, data sets with a larger diversity in these two dimensions are preferable. Our models based on supervised training with proxy outliers achieved rank three in Task 2 of the DCASE2020 Challenge.

==> lrgscy.tex <==
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}{.20\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{img/data_categories.png}
        \caption{Data Kinds}
        \label{fig:data_kinds}
    \end{subfigure}\hspace{0.5cm}
    \begin{subfigure}{.20\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{img/supervised_setting.png}
        \caption{Supervised Setting}
        \label{fig:supervised_setting}
    \end{subfigure}\hspace{0.5cm}
    \begin{subfigure}{.20\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{img/unsupervised_setting.png}
        \caption{Unsupervised Setting}
        \label{fig:unsupervised_setting}
    \end{subfigure}\hspace{0.5cm}
    \begin{subfigure}{.20\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{img/outlier_exposed_setting.png}
        \caption{Unrelated Sounds Setting}
        \label{fig:our_setting}
    \end{subfigure}
    \caption{Sub-figure \ref{fig:data_kinds} depicts the three types of data for machine condition monitoring. Normal and anomalous sounds are emitted by the target machine in normal, anomalous state, respectively. Unrelated sounds are all other sounds in the audio domain, excluding normal and anomalous sounds of the target machine. Sub-figures \ref{fig:supervised_setting}, \ref{fig:unsupervised_setting}, and \ref{fig:supervised_setting} show the data used in the supervised, unsupervised, and unrelated anomaly detection setting, respectively. Dark grey area represents the negative, light grey area the positive class. Samples in the withe area are not available/ used.}
    %Although the classical supervised setting would be optimal, real anomalies are rare and/ or expensive to collect.}
    \label{fig:settings}
\end{figure*}

\begin{table}[t!]

    \centering
    \begin{tabular}{l l l l}
    Name & \makecell{recording\\conditions} & \makecell{recording \\ condition \\ variation} &\makecell{content\\type} \\ \hline
    same type       & equal     & none      & same machine type only \\
    different types & equal     & none      & different machine types  \\
    all types       & equal     & none      & all machine types \\
    other MCM set   & different & none      & all machine tyse \\
    TAU ASC         & different & small\\
    AudioSet        & different & large \\
    
    \end{tabular}
    \caption{}
    \label{tab:unrelated_data}
\end{table}

\begin{table}[t!]

    \centering
    \begin{tabular}{ @{}lcccclc@{} }
    %\toprule
    \multicolumn{4}{c}{ResNet} & & \multicolumn{2}{c}{Residual Block (RB)}\\
    \cmidrule(lr{.5em}){1-4} \cmidrule(lr{.5em}){6-7} 
    Type & \#K & KS 1 & KS 2 & & Type & KS\\
    \cmidrule(lr{.5em}){1-4} \cmidrule(lr{.5em}){6-7} 
    Conv        & $64$      & $5$ &     & & Conv        & KS 1  \\
    BN          & -         & -   &     & & BN          &       \\
    RB          & $64$      & $3$ & $1$ & & Conv        & KS 2  \\
    Max Pool    & -         & $2$ & -   & & BN          &       \\
    RB          & $64$      & $3$ & $3$ & & Add Input   &    \\
    Max Pool    & -         & $2$ & -   & & \\
    RB          & $64$      & $3$ & $3$ & & \\
    RB          & $64$      & $3$ & $1$ & & \\
    Max Pool    & -         & $2$ & -   & & \\
    RB          & $128$     & $1$ & $1$ & & \\
    RB          & $256$     & $1$ & $1$ & & \\
    RB          & $256$     & $1$ & $1$ & & \\
    Conv        & $256$     & $1$ & -   & & \\
    BN          & -         & -   & -   & & \\
    GAP         & -         & -   & -   & & \\
    %\bottomrule
    \end{tabular}
    \caption{Model architecture by Koutini et al.~\cite{Koutini_2019}. \#K and KS are the number of kernels and kernel size, respectively. Residual Blocks (RB) consist of two Convolutional (Conv) layers with \#K kernels, each followed by a Batch Normalization (BN) layer. GAP is a Global Average Pooling Layer. We use ReLU non-linearities.}
    \label{tab:resnet}
\end{table}


